Measuring Discrete Sensing Capability for ISAC via Task Mutual Information

6G technology offers a broader range of possibilities for communication systems to perform ubiquitous sensing tasks, including health monitoring, object recognition, and autonomous driving. Since even minor environmental changes can significantly degrade system performance, and conducting long-term posterior experimental evaluations in all scenarios is often infeasible, it is crucial to perform a priori performance assessments to design robust and reliable systems. In this paper, we consider a discrete ubiquitous sensing system where the sensing target has \(m\) different states \(W\), which can be characterized by \(n\)-dimensional independent features \(X^n\). This model not only provides the possibility of optimizing the sensing systems at a finer granularity and balancing communication and sensing resources, but also provides theoretical explanations for classical intuitive feelings (like more modalities and more accuracy) in wireless sensing. Furthermore, we validate the effectiveness of the proposed channel model through real-case studies, including person identification, displacement detection, direction estimation, and device recognition. The evaluation results indicate a Pearson correlation coefficient exceeding 0.9 between our task mutual information and conventional experimental metrics (e.g., accuracy). The open source address of the code is: https://github.com/zaoanhh/DTMI

==> fig/model_fig.tex <==
\makeatletter


% helper macro
\newcommand\tikz@expand@dimen[2]{\tikzset{minimum #2=#1}}
% tikz styles: adjust min width/height of nodes
\tikzset{
	add dimen/.code 2 args={%
			\pgfkeysgetvalue{/pgf/minimum #1}\tikz@dimen@min
			\expandafter\tikz@expand@dimen\expandafter{\tikz@dimen@min + #2 * 2em}{#1}%
		},
	wider/.style={add dimen={width}{#1}},
	higher/.style={add dimen={height}{#1}},
}
\makeatother
\def \globalscale {1.000000}
\def\linewidthEz {0.6pt}
\begin{tikzpicture}[y=1cm, x=1cm, yscale=\globalscale,xscale=\globalscale, inner sep=0pt, outer sep=0pt,meta box/.style={
				draw,
				black,
				very thick,
				text centered
			},
		punkt/.style={
				meta box,
				rectangle,
				rounded corners,
				inner sep=5pt,
				minimum height=0.2em,
				minimum width=0.2em,
				align=center
			},
		round box/.style={
				meta box,
				circle
			},
		every fit/.style={
				draw,
				thick,
				inner sep=6pt
			}]

	\tikzstyle{myarrow}=[line width=1pt,-{Stealth[round]}]


	\coordinate (Fig_left) at (0,0);

	\node[punkt] (task_node) at (Fig_left) {Status\\ {\color{myNewColorA}$\mathcal{W}$}};

    \node[punkt,right=0.7cm of task_node] (x) {Feature\\ {\color{myNewColorA}$\mathcal{X}^n$}};

    \node[punkt,right=1.5cm of x] (y) {Sensing Space\\ {\color{myNewColorA}$\mathcal{Y}^n$}};

    \node[punkt,right=1cm of y] (hat_W) {Result\\ {\color{myNewColorA}$\hat{\mathcal{W}}$}};

    \draw[myarrow] (task_node.east) to node[above=0.1]{$w$} (x.west);

    \draw[myarrow] (x.east) to node[above=0.1]{$p(y^n|x^n)$} (y.west);

    \draw[myarrow] (y.east) to node[above=0.1]{$g(y^n)$} (hat_W.west);




\end{tikzpicture}

==> fig/vn.tex <==
\begin{tikzpicture}
    % Define the sets
    \def\firstset{(0,0) ellipse (2.5cm and 1.5cm)}
    \def\secondset{(2.5,0) ellipse (2.5cm and 1.5cm)}
    % Fill the sets
    \draw[fill=white!30] \firstset node[align=left,xshift=-30] {$|A_{\varepsilon}^n(X^n)|$\\ $\approx 2^{\sum_{i=1}^n H(X_i)}$};
    \draw[fill=white!30] \secondset node[align=left,xshift=30] {$|A_{\varepsilon}^n(Y^n)|$\\ $\approx 2^{\sum_{i=1}^n H(Y_i)}$};
    % Calculate the intersection
    \begin{scope}
        \clip \firstset;
        \fill[myNewColorC] \secondset;
    \end{scope}
    % Draw the sets' outlines
    \draw \firstset node {};
    \draw \secondset node {};
    % Draw the intersection label
    \node[align=left,text=myNewColorA] at (1.25,2) {$|B_{\varepsilon}^n| \approx 2^{\sum_{i=1}^n H(X_i,Y_i)}$};
    \draw (1.3,0.7) -- (1.8,1.8);
\end{tikzpicture}

==> sections/intro-0514.tex <==
\section{Introduction}
The recent development of next-generation (5G-Advanced and 6G) communication technology motivates the integrated sensing and communication (ISAC) studies from various perspectives, such as the localization models~\cite{sayed2005network, shen2010fundamental, wang2018device}, the power and sub-channel allocation algorithms~\cite{phunchongharn2013resource, zhang2017network}, the dual-functional waveforms design~\cite{zhang2024dual} and so on.
ISAC has been conceptualized, designed, and optimized for making communication and sensing functions complementary to each other.

% \addtolength{\topmargin}{0.161in}

However, the goal of wireless communication is to minimize the impact of channel noise within the Shannon’s limit, while the goal of wireless sensing is to utilize the channel noise and then to identify the entities or the corresponding nature of the channel.
The different goals bring the inherent trade-off between communication and sensing performance when integrating them together.
To better address such resource competition from each other, it is essential to quantify the ability to communicate and sense under a given channel.
The communication aspects can be bounded by Shannon's theorem, but the sensing part lacks unified and efficient theory support.
Existing work on sensing theory suffers from deficiencies in different aspects, such as limited applicable tasks~\cite{shen2010fundamental} and incomplete evaluation metrics~\cite{zhang2024dual, phunchongharn2013resource}.
%which is fundamentally caused by the lack of \textit{quantitative analysis of the sensing capacity}.

 
%In particular, sensing capability is the upper bound of accuracy in restoring the sensed object from a given wireless signal.
In the present paper, we will theoretically analyze the sensing capability and measure it based channel encoder model.
% propose a corresponding channel model.
The core problem of wireless sensing is that of reproducing via the interfered signals at the receiver either exactly or approximately the interfering source, considered as the sensed object.
As illustrated in Fig~\ref{fig:intro}, the ISAC system can be formulated by $\mathbf{Y}=\mathbf{H}\mathbf{X}+\mathbf{N}$, where $\mathbf{Y}$ is the received signal, $\mathbf{X}$ is the transmitted signal, $\mathbf{H}$ is the channel status, and $\mathbf{N}$ is the noise that might be introduced by sensed objects.

% \begin{figure}
%     \includegraphics[width=\linewidth]{inreo-new.pdf}
%     \caption{Schematic diagram of a general ISAC system.}
%     \label{fig:intro}
% \end{figure}



Intuitively, the system sensing capability can be evaluated by analyzing how the received signals reflect the channel status, such as sensing mutual information $I(\mathbf{H};\mathbf{Y})$~\cite{liu2021cramer,zhang2021overview}.
But it doesn’t work well for the following two reasons.
First, it is difficult to obtain complete information about the signal itself, we can only identify the sensory objects by analyzing several received signal features, such as the time-of-arrival (TOA), angle-of-arrival (AOA) and received signal strength (RSS). The relationship between the sensing capability of such features and the signal itself is ambiguous.
For example, when containing the same level of noise, the AoA estimation error is related to the orientation of the antenna array~\cite{tai2019toward}, as shown in Fig~\ref{fig:aoa_mapfi}.
Second, frequently the sensed objects have various types, including moving entities placed in the channel, temperature or humidity fields affecting the channel, etc. The sensing capability analysis must be designed to operate for all possible types, not just the one that will actually be chosen since this is unknown at the time of design. 



Fortunately, if the number of signal features and object types in the sets is finite, then the monotone function of the mapping between them can be regarded as a measure of the sensing capability when the pair is chosen from the sets.
The most natural choice of such a monotone function is still mutual information for various reasons:

\begin{enumerate}
    \item It is suitable to the communication theorem and thus easier to integrate. The ultimate goal of sensing capability assessment is to provide an optimization basis for the trade-off between communication and sensing in ISAC systems so that entropy-based methods can achieve calculations more efficiently.
    \item  It evaluates the amount of information contained in one random variable about another random variable, which is nearer to our intuitive feeling as to the proper measure for sensing: how much information is obtained in the observed signal features about the sensed object.
\end{enumerate}

In this paper, we propose a general sensing channel encoder model to help determine the sensing capability -- the upper bound and lower bound of error in restoring the sensed object from given wireless signal features.
Main contributions are as following:

\begin{figure}[t]
    \centering
    \includegraphics[width=0.6\linewidth]{mapfi.pdf}
    \caption{Due to the nonlinear relationship between AoA and the phase change of received signals, even with comparable capabilities in estimating channel responses, there can still be order-of-magnitude differences in the estimation error of AoA when the orientation of the antenna array varies..}
    \label{fig:aoa_mapfi}
\end{figure}

\begin{itemize}
    \item We propose a sensing channel encoder model to describe the sensing system, and derive the fundamental limits of specific sensing objects under given signal features, in terms of a performance measure called \textit{discrete task mutual information} (DTMI). This approach unifies such information from different features in a canonical form as a weighted sum associated with the weights characterizing the information intensity.
    \item Based on DTMI, we first provide upper and lower bounds of sensing errors for ubiquitous sensing systems and give a sufficient condition for lossless sensing. It enhances the interpretability of current sensing systems and can be further used to guide the problem of resource allocation for communication and sensing in ISAC systems.
    \item We validate the effectiveness of the proposed sensing system model in several real-world cases, including binary classification tasks such as Wi-Fi-based human identification and RFID-based displacement detection, and multi-classification tasks such as direction sensing based on electromagnetic signals and device identification based on traffic features. The experiment results show that the consistency between our proposed sensing capability evaluation method and the actual task results is up to 0.9 (Pearson correlation coefficient).
\end{itemize}

The rest of the paper is organized as follows. Section~\ref{sec:related} reviews the related work. 
We introduce the sensing channel encoder model in Section~\ref{sec:model}.
In Section~\ref{sec:corollary}, we give a theoretical explanation for some classical phenomena in sensing systems.
Finally, we evaluate its performance in real examples in Section~\ref{sec:case}.

==> sections/intro.tex <==
\section{Introduction}
% \IEEEPARstart{T}{he} development of random wireless communication technology, higher frequency bands (millimeter waves and even terahertz), wider bandwidths, and larger antenna arrays make high-precision and high-resolution sensing possible, thus enabling Integrated Sensing and Communication in one system (ISAC), making communication and perception functions complementary to each other.

\IEEEPARstart{I}{ntegrated} sensing and communication (ISAC) has been conceptualized, designed, and optimized for the goal of making communication and sensing functions complementary to each other.
To affiliate this, Shannon’s limit provides a fundamental theorem on the aspect of  communication, while the theoretical analysis for sensing-related design and implementation is  not enough.
Particularly, wireless sensing has long been plagued by a lack of theoretical limits, usually in the form of missing capacity metrics.
For example, 

Thanks to the ubiquitous nature of signals and the cheap and easy deployment of transceiver terminals, wireless sensing technology is highly favored against the background of the booming development of the intelligent Internet of Things.
In the past ten years, a large number of wireless sensing applications have emerged~\cite{liu2022survey,ma2019wifi,fang2015multi,yang2019review}.
Many researchers try to build wireless sensing systems based on wireless signals, such as sound signals, WiFi signals, LTE signals, etc., to complete sensing tasks, including target positioning~\cite{shangTameraContactlessCommodity2023,yangSeeWallsCOTS2015}, material identification~\cite{liangFGLiquIDContactlessFinegrained2021,yanWipainterFinegrainedMaterial2024}, health monitoring~\cite{adibSmartHomesThat2015,zhangVeCareStatisticalAcoustic2023}, etc.


However, current analysis of perception system performance often relies on experimental evaluation and lacks theoretical evaluation indicators (similar to channel capacity, mutual information, etc. in communication).
Since fine-grained experimental evaluation for multiple situations in a large number of scenarios is difficult, it is difficult to determine how to allocate resources (e.g., bandwidth) for perception and communication in a ISAC system that is reasonable enough.
For a typical ISAC system, $Y=HX+N$, where $Y$ is the receiving signal, $X$ is the transmitting signal, $H$ is the channel state response, and $N$ is the noise.
We usually use perceptual mutual information $I(H;Y)$ to represent its perception ability.
However, the level of estimation of the channel state response $H$ is not entirely equivalent to the performance of the sensing system.
For example, in position sensing, a very typical sensing feature is the angle of arrival (AoA) of the signal.
{\color{red} Relevant studies}~\cite{tai2019toward} have shown that when containing the same level of noise, the AoA estimation error is related to the orientation of the antenna array.
As shown in Fig.~\ref{fig:aoa}, the closer the arrival angle is to 90 degrees, the smaller the estimation error is.

\begin{figure}
    \includegraphics[width=\linewidth]{mapfi.pdf}
    \caption{The AoA estimation error with the different orientations of antenna arrays.}
    \label{fig:aoa}
\end{figure}

\begin{figure}
    \includegraphics[width=\linewidth]{pre.pdf}
    \caption{There is a strong correlation between mutual information and estimation error.}
    \label{fig:aoa2}
\end{figure}
In this paper, we propose discrete task mutual information (DTMI) to evaluate the dependence between discrete sensing task states $W$ and sensing features $F$ extracted from the signal.

\textbf{Contributions:}
\begin{itemize}
    {\color{red} \item We propose a new evaluation indicator, discrete task mutual information (DTMI), to evaluate the performance of the sensing system.
    \item We analyze the relationship between the DTMI and the sensing system performance.
    \item We propose a method to optimize the sensing system based on the DTMI.}
\end{itemize}
